Pauli Gadget Synthesis for Gatesets with Arbitrary Even Arity Clifford Gates

We propose an algorithm that can synthesize circuits to gate sets consisting of a 2n-arity Clifford gate and arbitrary single qubit rotations. To do this, we represent the circuit as a sequence of Pauli gadgets and jointly synthesize them by placing the multi-qubit Clifford in the synthesized circuit and pushing its adjoint through the remaining gadgets such that some qubits are disconnected from some gadgets. The pushed gadgets are collected in a Clifford tableau, which is decomposed afterwards. With the help of our algorithm we run experiments where we synthesize circuits to varying sizes of target multi-qubit gates. These experiments indicate that increases in gate size can lead to smaller output circuits, and that different connectivity constraints have meaningful differences in how higher arity gates effect the circuit sized.

==> eptcsdata.tex <==
\providecommand{\firstpage}{18}
\providecommand{\publicationstatus}{J. van de Wetering, O. Oreshkov, and A.B. Sainz (Eds.):\\
Quantum Physics and Logic 2026 (QPL 2026)\\
EPTCS 456, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.456.2}{10.4204/EPTCS.456.2}}
\pdfoutput=1

